Proof nets for the Lambek-Grishin calculus

Grishin's generalization of Lambek's Syntactic Calculus combines a non-commutative multiplicative conjunction and its residuals (product, left and right division) with a dual family: multiplicative disjunction, right and left difference. Interaction between these two families takes the form of linear distributivity principles. We study proof nets for the Lambek-Grishin calculus and the correspondence between these nets and unfocused and focused versions of its sequent calculus.

==> pnmacros.tex <==

 \newcounter{myovalx}
 \newcounter{myovaly}
 \newcounter{myovalz}
 \newcounter{myovalxx}
 \newcounter{myovalyy}
 \newcounter{myovalzz}

 \newcounter{circlex}
 \newcounter{circley}

 \newcounter{dotfactor}
 \setcounter{dotfactor}{2}

\newenvironment{proofnet}{\renewcommand{\tabcolsep}{0pt}
 \renewcommand{\arraystretch}{0}
 \setlength{\unitlength}{\bre}}{}

\newcommand{\ltagz}{\ensuremath{\text{LTAG}_0}}
\newcommand{\ltag}{\mbox{LTAG}}
\newcommand{\nldr}{\textbf{NL}\Diamond_{\calr}}
\newcommand{\nldrm}{\textbf{NL}\Diamond_{\calr^{-}}}
\newcommand{\conbox}{\stackrel{\sqcap}{\rule{0pt}{2pt}}\!}
\newcommand{\debox}{\stackrel{\sqcup}{\rule{0pt}{2pt}}\!}
\newcommand{\condia}{\stackrel{\wedge}{\rule{0pt}{2pt}}\!}
\newcommand{\dedia}{\stackrel{\vee}{\rule{0pt}{2pt}}\!}
\newcommand{\editout}[1]{}
\newcommand{\myfilltype}{}
\newcommand{\filledcircleindex}[4]{%
         \filledcircle{#1}{#2}{#3}%
         \circleindex{#1}{#2}{\scriptstyle #4}}
\newcommand{\filledcircle}[3]{%
         \put(#1,#2){\circle*{#3}}}%
\newcommand{\circleindex}[3]{%
         \put(#1,#2){\makebox(0,0){\ensuremath{\color{white}\boldsymbol{#3}}}}}
\newcommand{\bang}{!}
\newcommand{\dl}[3]{#2 \backslash_{#1} #3}   
\newcommand{\dr}[3]{#2 /_{#1} #3}   
\newcommand{\p}[3]{#2 \circ_{#1} #3}
\renewcommand{\l}[2]{#2^{\triangleleft_{#1}}}   
\renewcommand{\r}[2]{#2^{\triangleright_{#1}}}   
\newcommand{\zip}[2]{\langle #2 \rangle^{#1}}   
\newcommand{\unzip}[2]{\lfloor #2 \rfloor^{#1}} 
\newcommand{\unpack}[2]{\lceil #2 \rceil^{#1}}
\newcommand{\cotensor}{\mathbin{\circ}}
\newcommand{\tensor}{\mathbin{\bullet}}

\newcommand{\sys}[1]{\ensuremath{\bf #1}}
\newcommand{\weg}[1]{}

\newcommand{\one}{\boldsymbol{1}}
\newcommand{\zero}{\boldsymbol{0}}

\newcommand{\yinitial}[2]{\initial{2}{{\Huge #1}\hspace{.4ex}}{\scshape #2}}
%\def\yinitial#1
%{\font\yinit=yinit scaled 800
%zero_depth:=false
%\hangindent=0.5cm
%\hangafter=-4
%\hskip-0.0cm
%\lower9.7mm
%\hbox{\yinit #1}
%\hskip1.5mm}

\newcommand{\pnoval}[6]{%
 \setcounter{myovalx}{#1+1}%
 \setcounter{myovaly}{#3+#6-1}%
 \setcounter{myovalxx}{#1+#5-1}%
 \setcounter{myovalyy}{#3+1}%
 \qbezier(\themyovalx.#2,#3.#4)(#1.#2,#3.#4)(#1.#2,\themyovalyy.#4)
 \drawline(#1.#2,\themyovaly.#4)(#1.#2,\themyovalyy.#4)
 \setcounter{myovalyy}{#3+#6}%
 \qbezier(#1.#2,\themyovaly.#4)(#1.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovalyy.#4)
 \drawline(\themyovalx.#2,\themyovalyy.#4)(\themyovalxx.#2,\themyovalyy.#4)
 \setcounter{myovalx}{#1+#5}%
 \setcounter{myovalyy}{#3+1}%
 \drawline(\themyovalx.#2,\themyovaly.#4)(\themyovalx.#2,\themyovalyy.#4)
 \qbezier(\themyovalx.#2,\themyovalyy.#4)(\themyovalx.#2,#3.#4)(\themyovalxx.#2,#3.#4)
 \setcounter{myovalyy}{#3+#6}%
 \qbezier(\themyovalxx.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovaly.#4)
}

\newcommand{\pnovald}[6]{%
 \setcounter{myovalx}{#1+1}%
 \setcounter{myovaly}{#3+#6-1}%
 \setcounter{myovalxx}{#1+#5-1}%
 \setcounter{myovalyy}{#3+1}%
 \qbezier(\themyovalx.#2,#3.#4)(#1.#2,#3.#4)(#1.#2,\themyovalyy.#4)
 \drawline(#1.#2,\themyovaly.#4)(#1.#2,\themyovalyy.#4)
 \setcounter{myovalyy}{#3+#6}%
 \qbezier(#1.#2,\themyovaly.#4)(#1.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovalyy.#4)
 \setcounter{myovalyy}{#3}%
 \drawline(\themyovalx.#2,\themyovalyy.#4)(\themyovalxx.#2,\themyovalyy.#4)
 \setcounter{myovalx}{#1+#5}%
 \setcounter{myovalyy}{#3+1}%
 \drawline(\themyovalx.#2,\themyovaly.#4)(\themyovalx.#2,\themyovalyy.#4)
 \qbezier(\themyovalx.#2,\themyovalyy.#4)(\themyovalx.#2,#3.#4)(\themyovalxx.#2,#3.#4)
 \setcounter{myovalyy}{#3+#6}%
 \qbezier(\themyovalxx.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovaly.#4)
}

\newcommand{\pnovallr}[6]{%
 \setcounter{myovalx}{#1+1}%
 \setcounter{myovaly}{#3+#6-1}%
 \setcounter{myovalxx}{#1+#5-1}%
 \setcounter{myovalyy}{#3+1}%
 \qbezier(\themyovalx.#2,#3.#4)(#1.#2,#3.#4)(#1.#2,\themyovalyy.#4)
 \drawline(#1.#2,\themyovaly.#4)(#1.#2,\themyovalyy.#4)
 \setcounter{myovalyy}{#3+#6}%
 \qbezier(#1.#2,\themyovaly.#4)(#1.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovalyy.#4)
 \setcounter{myovalyy}{#3}%
 \setcounter{myovalx}{#1+#5}%
 \setcounter{myovalyy}{#3+1}%
 \drawline(\themyovalx.#2,\themyovaly.#4)(\themyovalx.#2,\themyovalyy.#4)
 \qbezier(\themyovalx.#2,\themyovalyy.#4)(\themyovalx.#2,#3.#4)(\themyovalxx.#2,#3.#4)
 \setcounter{myovalyy}{#3+#6}%
 \qbezier(\themyovalxx.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovalyy.#4)(\themyovalx.#2,\themyovaly.#4)
}
%\newcommand{\rectangle}[2]{}
\newcommand{\rectangle}[2]{%
 \rule{#1\unitlength}{#2\unitlength}}
\newcommand{\mycput}[1]{%
 \makebox(0,0){#1}}
\newcommand{\cmput}[1]{%
 \makebox(0,0){\ensuremath{#1}}}
\newcommand{\lp}{\textbf{LP}}
\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}
%\newcommand{\qed}{\hfill $\Box$ \vspace{3mm}}
\newcommand{\bo}{[}
\newcommand{\bc}{]}
\newcommand{\bs}{\backslash}
\newcommand{\Gammap}{\Gamma^{\prime}}

\newcommand{\ra}{\vdash\rule{0mm}{0.6em}}
\newcommand{\rr}{\twoheadrightarrow}
\newcommand{\reduce}[2]{\ensuremath{#1 \rightarrow #2}}   

\newcommand{\xdots}{\raisebox{1.2ex}{$\cdots$}}
\newcommand{\ydots}{\raisebox{.2ex}{$\cdots$}}
\newcommand{\rbp}[1]{\raisebox{1ex}{$#1$}}

\newcommand{\con}[1]{\textup{#1}}   
\newcommand{\pn}[1]{{\cal #1}}   
\newcommand{\Boxd}{\Box^{\downarrow}}
\newcommand{\ax}[1]{\infer[\bo Ax\bc]{#1 \ra\rule{0mm}{0.6em} #1}{}}
\newcommand{\axv}[1]{\infer[\bo Ax\bc]{#1 \vdash\rule{0mm}{0.6em} #1}{}}
\newcommand{\pair}[2]{\langle #1 , #2 \rangle}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\etc}{etc.\@\xspace}

% = equilateral tensor lines

\newcommand{\bottomcentertotopright}{%
   \drawline(2.4,0.69282032)(3.6,2.7712813)}
\newcommand{\bottomcentertotopleft}{%
   \drawline(1.6,0.69282032)(0.4,2.7712813)}
\newcommand{\toplefttotopright}{%
   \drawline(0.8,3.4641016)(3.2,3.4641016)}
\newcommand{\topcentertobottomright}{%
   \drawline(2.4,2.7712813)(3.6,0.69282032)}
\newcommand{\topcentertobottomleft}{%
   \drawline(1.6,2.7712813)(0.4,0.69282032)}
\newcommand{\bottomlefttobottomright}{%
   \drawline(0.8,0)(3.2,0)}

% = equilateral par lines

\newcommand{\topcentertobottomrightd}{%
   \dottedline{.\thedotfactor}(2.4,2.7712813)(3.6,0.69282032)}
\newcommand{\topcentertobottomleftd}{%
   \dottedline{.\thedotfactor}(1.6,2.7712813)(0.4,0.69282032)}
\newcommand{\bottomlefttobottomrightd}{%
   \dottedline{.\thedotfactor}(0.8,0)(3.2,0)}
\newcommand{\bottomcentertotoprightd}{%
   \dottedline{.\thedotfactor}(2.4,0.69282032)(3.6,2.7712813)}
\newcommand{\bottomcentertotopleftd}{%
   \dottedline{.\thedotfactor}(1.6,0.69282032)(0.4,2.7712813)}
\newcommand{\toplefttotoprightd}{%
   \dottedline{.\thedotfactor}(0.8,3.4641016)(3.2,3.4641016)}

% = connectors for the different pairs of par lines

\newcommand{\bottomcenterconnect}{%
   \qbezier(1.6,0.69282032)(2,1.1)(2.4,0.69282032)}
\newcommand{\toprightconnect}{%
   \qbezier(3.6,2.7712813)(3.2,2.9641016)(3.2,3.4641016)}
\newcommand{\topleftconnect}{%
   \qbezier(0.4,2.7712813)(0.8,2.9641016)(0.8,3.4641016)}
\newcommand{\topcenterconnect}{%
   \qbezier(1.6,2.7712813)(2,2.3641016)(2.4,2.7712813)}
\newcommand{\bottomrightconnect}{%
   \qbezier(3.6,.69282032)(3.2,.5)(3.2,0)}
\newcommand{\bottomleftconnect}{%
   \qbezier(0.4,.69282032)(0.8,.5)(0.8,0)}

% = vectors tips for the tensor or par lines

\newcommand{\bottomcentertotoprightv}{%
   \drawline(3.6,2.7712813)(3.4133975,2.6480762)
   \drawline(3.6,2.7712813)(3.5866025,2.5480762)}
\newcommand{\bottomcentertotopleftv}{%
   \drawline(0.4,2.7712813)(0.58660254,2.6480762)
   \drawline(0.4,2.7712813)(0.41339746,2.5480762)}
\newcommand{\toprighttobottomcenterv}{%
   \drawline(2.4,0.69282032)(2.5866025,0.8160254)
   \drawline(2.4,0.69282032)(2.4133975,0.9160254)}
\newcommand{\toplefttobottomcenterv}{%
   \drawline(1.6,0.69282032)(1.4133975,0.8160254)
   \drawline(1.6,0.69282032)(1.5866025,0.9160254)}
\newcommand{\toplefttotoprightv}{%
   \drawline(3.2,3.4641016)(3.0,3.3641016)
   \drawline(3.2,3.4641016)(3.0,3.5641016)}
\newcommand{\toprighttotopleftv}{%
   \drawline(0.8,3.4641016)(1.0,3.3641016)
   \drawline(0.8,3.4641016)(1.0,3.5641016)}
\newcommand{\topcentertobottomrightv}{%
   \drawline(3.6,0.69282032)(3.4133975,0.8160254)
   \drawline(3.6,0.69282032)(3.5866025,0.9160254)}
\newcommand{\bottomrighttotopcenterv}{%
   \drawline(2.4,2.7712813)(2.5866025,2.6480762)
   \drawline(2.4,2.7712813)(2.4133975,2.5480762)}
\newcommand{\topcentertobottomleftv}{%
   \drawline(0.4,0.69282032)(0.58660254,0.8160254)
   \drawline(0.4,0.69282032)(0.41339746,0.9160254)}
\newcommand{\bottomlefttotopcenterv}{%
   \drawline(1.6,2.7712813)(1.4133975,2.6480762)
   \drawline(1.6,2.7712813)(1.5866025,2.5480762)}
\newcommand{\bottomlefttobottomrightv}{%
   \drawline(3.2,0)(3.0,0.1)
   \drawline(3.2,0)(3.0,-0.1)}
\newcommand{\bottomrighttobottomleftv}{%
   \drawline(0.8,0)(1.0,0.1)
   \drawline(0.8,0)(1.0,-0.1)}

% = par links

\newcommand{\partopcenter}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \topcentertobottomrightd
  \topcentertobottomleftd
  \topcenterconnect
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\parbottomcenter}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} } 
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \bottomcentertotoprightd
  \bottomcentertotopleftd
  \bottomcenterconnect
  \put(2,2.3094011){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\partopleft}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#3}} }
  \bottomcentertotopleftd
  \toplefttotoprightd
  \topleftconnect
  \put(2,2.3094011){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\parbottomleft}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \topcentertobottomleftd
  \bottomlefttobottomrightd
  \bottomleftconnect
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\partopright}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#4}} }
  \bottomcentertotoprightd
  \toplefttotoprightd
  \toprightconnect
  \put(2,2.3094011){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\parbottomright}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#4}} }
  \topcentertobottomrightd
  \bottomlefttobottomrightd
  \bottomrightconnect
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}

% = tensor links

\newcommand{\tensortopcenter}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \topcentertobottomright
  \topcentertobottomleft
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\tensorbottomcenter}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \bottomcentertotopright
  \bottomcentertotopleft
  \put(2,2.3094011){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\tensortopleft}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#3}} }
  \bottomcentertotopleft
  \toplefttotopright
  \put(2,2.3094011){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\tensorbottomleft}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \topcentertobottomleft
  \bottomlefttobottomright
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\tensortopright}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#4}} }
  \bottomcentertotopright
  \toplefttotopright
  \put(2,2.3094011){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}
\newcommand{\tensorbottomright}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#4}} }
  \topcentertobottomright
  \bottomlefttobottomright
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \end{picture}}}

% = centered par links

\newcommand{\parc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{2}{2.3094011}{.8}{#1}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \end{picture}}}
\newcommand{\parbottomc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  % outgoing lines at 120 degrees from circle
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)%
  % arrow
  \drawline(2,0.8)(1.9,1)
  \drawline(2,0.8)(2.1,1)
  \end{picture}}}
\newcommand{\parunitb}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{2}{1.7320508}{.8}{#1}
  \drawline(2,2.1320508)(2,2.6641016)
  % arrow
  \drawline(2,2.6641016)(1.9,2.4641016)
  \drawline(2,2.6641016)(2.1,2.4641016)
  \end{picture}}}
\newcommand{\parunita}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{2}{1.7320508}{.8}{#1}
  \drawline(2,0.8)(2,1.3320508)
  % arrow
  \drawline(2,0.8)(1.9,1)
  \drawline(2,0.8)(2.1,1)
  \end{picture}}}

\newcommand{\parleftc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#3}} }
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(0.6,3.1176915)(0.81754265,3.1099565)
  \drawline(0.6,3.1176915)(0.712320508,2.9370133)
  \end{picture}}}
\newcommand{\parleftcb}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#3}} }
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(0.6,3.1176915)(0.81754265,3.1099565)
  \drawline(0.6,3.1176915)(0.712320508,2.9370133)
  \end{picture}}}
\newcommand{\parrightc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#4}} }
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(3.4,3.1176915)(3.1824573,3.1099565)
  \drawline(3.4,3.1176915)(3.2876795,2.9370133)
  \end{picture}}}
\newcommand{\parrightcb}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,0){\makebox(0,0){\ensuremath{#3}} }
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(3.4,3.1176915)(3.1824573,3.1099565)
  \drawline(3.4,3.1176915)(3.2876795,2.9370133)
  \end{picture}}}
\newcommand{\negparleftc}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(0.6,3.1176915)(0.81754265,3.1099565)
  \drawline(0.6,3.1176915)(0.712320508,2.9370133)
  \end{picture}}}
\newcommand{\negparleftcb}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(0.6,3.1176915)(0.81754265,3.1099565)
  \drawline(0.6,3.1176915)(0.712320508,2.9370133)
  \end{picture}}}
\newcommand{\negparrightc}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(3.4,3.1176915)(3.1824573,3.1099565)
  \drawline(3.4,3.1176915)(3.2876795,2.9370133)
  \end{picture}}}
\newcommand{\negparrightcb}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(4,3.4641016){\makebox(0,0){\ensuremath{#2}} }  
  \filledcircleindex{2}{2.3094011}{0.8}{#1}
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(3.4,3.1176915)(3.1824573,3.1099565)
  \drawline(3.4,3.1176915)(3.2876795,2.9370133)
  \end{picture}}}
\newcommand{\mparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \end{picture}}}
\newcommand{\mparbottomc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  % outgoing lines at 120 degrees from circle
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)%
  % arrow
  \drawline(2,2.6641016)(1.9,2.4641016)
  \drawline(2,2.6641016)(2.1,2.4641016)
  \end{picture}}}
\newcommand{\mparleftc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#4}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  % outgoing lines at 120 degrees from circle
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(0.6,0.34641012)(0.81754265,0.35414512)
  \drawline(0.6,0.34641012)(0.712320508,0.52708832)
  \end{picture}}}
\newcommand{\mparleftcb}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  % outgoing lines at 120 degrees from circle
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
%  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(0.6,0.34641012)(0.81754265,0.35414512)
  \drawline(0.6,0.34641012)(0.712320508,0.52708832)
  \end{picture}}}
\newcommand{\mnegparleftc}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#3}} }  
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  % outgoing lines at 120 degrees from circle
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(0.6,0.34641012)(0.81754265,0.35414512)
  \drawline(0.6,0.34641012)(0.712320508,0.52708832)
  \end{picture}}}
\newcommand{\mnegparleftcb}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }  
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  % outgoing lines at 120 degrees from circle
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(0.6,0.34641012)(0.81754265,0.35414512)
  \drawline(0.6,0.34641012)(0.712320508,0.52708832)
  \end{picture}}}
\newcommand{\mparrightc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#4}} }
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(3.4,0.34641012)(3.1824573,0.35414512)
  \drawline(3.4,0.34641012)(3.2876795,0.52708832)
  \end{picture}}}
\newcommand{\mnegparrightc}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){\ensuremath{#3}} }  
  \put(4,0){\makebox(0,0){\ensuremath{#2}} }  
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(3.4,0.34641012)(3.1824573,0.35414512)
  \drawline(3.4,0.34641012)(3.2876795,0.52708832)
  \end{picture}}}
\newcommand{\mnegparrightcb}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(4,0){\makebox(0,0){\ensuremath{#2}} }  
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(3.4,0.34641012)(3.1824573,0.35414512)
  \drawline(3.4,0.34641012)(3.2876795,0.52708832)
  \end{picture}}}
\newcommand{\mparrightcb}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(4,0){\makebox(0,0){\ensuremath{#2}} }  
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \filledcircleindex{2}{1.1547005}{0.8}{#1}
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(3.4,0.34641012)(3.1824573,0.35414512)
  \drawline(3.4,0.34641012)(3.2876795,0.52708832)
  \end{picture}}}
\newcommand{\partopcu}[3]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{0}{1.7320508}{0.8}{#1}
  \drawline(0,0.8)(0,1.3320508)
  \drawline(0,2.1320508)(0,2.6641016)
  \drawline(0,2.6641016)(-0.1,2.4641016)
  \drawline(0,2.6641016)(0.1,2.4641016)
  \end{picture}}}

\newcommand{\parbottomcu}[3]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \put(0,0){\makebox(0,0){\ensuremath{#2}} }
  \filledcircleindex{0}{1.7320508}{0.8}{#1}
  \drawline(0,0.8)(0,1.3320508)
  \drawline(0,2.1320508)(0,2.6641016)
  \drawline(0,0.8)(-0.1,1)
  \drawline(0,0.8)(0.1,1)
  \end{picture}}}

% = binary galois

\newcommand{\ttlparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #2 $} }  
  \put(4,0){\makebox(0,0){$ #4 $} }  
  \put(2,0){\makebox(0,0){$ #3 $} }
  \filledcircleindex{2}{1.1547005}{.8}{#1}
  \drawline(2,0.34641012)(2,0.7547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(0.6,0.34641012)(0.81754265,0.35414512)
  \drawline(0.6,0.34641012)(0.712320508,0.52708832)
  \end{picture}}}
\newcommand{\ttmparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #2 $} }  
  \put(4,0){\makebox(0,0){$ #4 $} }  
  \put(2,0){\makebox(0,0){$ #3 $} }
  \filledcircleindex{2}{1.1547005}{.8}{#1}
  \drawline(2,0.34641012)(2,0.7547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(2,0.34641012)(1.9,0.54641012)
  \drawline(2,0.34641012)(2.1,0.54641012)
  \end{picture}}}
\newcommand{\ttrparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #2 $} }  
  \put(4,0){\makebox(0,0){$ #4 $} }  
  \put(2,0){\makebox(0,0){$ #3 $} }
  \filledcircleindex{2}{1.1547005}{.8}{#1}
  \drawline(2,0.34641012)(2,0.7547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \drawline(3.4,0.34641012)(3.1824573,0.35414512)
  \drawline(3.4,0.34641012)(3.2876795,0.52708832)
  \end{picture}}}

% = binary dual galois

\newcommand{\tmlparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #2 $}}  
  \put(4,3.4641016){\makebox(0,0){$ #4 $}}  
  \put(2,3.4641016){\makebox(0,0){$ #3 $}}
  \filledcircleindex{2}{2.30940111}{.8}{#1}
  \drawline(2,3.1176915)(2,2.7094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(0.6,3.1176915)(0.81754265,3.1099565)
  \drawline(0.6,3.1176915)(0.712320508,2.9370133)
  \end{picture}}}
\newcommand{\tmmparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #2 $}}  
  \put(4,3.4641016){\makebox(0,0){$ #4 $}}  
  \put(2,3.4641016){\makebox(0,0){$ #3 $}}
  \filledcircleindex{2}{2.30940111}{.8}{#1}
  \drawline(2,3.1176915)(2,2.7094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(2,3.1176915)(1.9,2.9176915)
  \drawline(2,3.1176915)(2.1,2.9176915)
  \end{picture}}}
\newcommand{\tmrparc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #2 $}}  
  \put(4,3.4641016){\makebox(0,0){$ #4 $}}  
  \put(2,3.4641016){\makebox(0,0){$ #3 $}}
  \filledcircleindex{2}{2.30940111}{.8}{#1}
  \drawline(2,3.1176915)(2,2.7094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \drawline(3.4,3.1176915)(3.1824573,3.1099565)
  \drawline(3.4,3.1176915)(3.2876795,2.9370133)
  \end{picture}}}

% = centered tensor link

\newcommand{\tensorc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #3 $} }  
  \put(4,0){\makebox(0,0){$ #4 $} }  
  \put(2,3.4641016){\makebox(0,0){$ #2 $} }
  \put(2,1.1547005){\circle{.8}}
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \end{picture}}}
\newcommand{\tensorcl}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #3 $} }  
  \put(2,3.4641016){\makebox(0,0){$ #2 $} }
  \put(2,1.1547005){\circle{.8}}
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \end{picture}}}
\newcommand{\tensorcr}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(4,0){\makebox(0,0){$ #3 $} }  
  \put(2,3.4641016){\makebox(0,0){$ #2 $} }
  \put(2,1.1547005){\circle{.8}}
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,2.6641016)(2,1.5547005)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \end{picture}}}
\newcommand{\mtensorc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #3 $}}  
  \put(4,3.4641016){\makebox(0,0){$ #4 $}}  
  \put(2,0){\makebox(0,0){$ #2 $}}
  \put(2,2.3094011){\circle{.8}}
  \put(2,2.30940111){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \end{picture}}}
\newcommand{\mtensorcright}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(4,3.4641016){\makebox(0,0){$ #3 $}}  
  \put(2,0){\makebox(0,0){$ #2 $}}
  \put(2,2.3094011){\circle{.8}}
  \put(2,2.30940111){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \end{picture}}}
\newcommand{\mtensorcleft}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #3 $}}  
  \put(2,0){\makebox(0,0){$ #2 $}}
  \put(2,2.3094011){\circle{.8}}
  \put(2,2.30940111){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,0.8)(2,1.9094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \end{picture}}}
\newcommand{\ttensorc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #2 $} }  
  \put(4,0){\makebox(0,0){$ #4 $} }  
  \put(2,0){\makebox(0,0){$ #3 $} }
  \put(2,1.1547005){\circle{.8}}
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,0.34641012)(2,0.7547005)
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \end{picture}}}
\newcommand{\tmtensorc}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #2 $}}  
  \put(4,3.4641016){\makebox(0,0){$ #4 $}}  
  \put(2,3.4641016){\makebox(0,0){$ #3 $}}
  \put(2,2.3094011){\circle{.8}}
  \put(2,2.30940111){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,3.1176915)(2,2.7094011)
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \end{picture}}}

\newcommand{\negtensora}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){$ #2 $} }  
  \put(4,0){\makebox(0,0){$ #3 $} }  
  \put(2,1.1547005){\circle{.8}}
  \put(2,1.1547005){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(0.6,0.34641012)(1.6535989,0.95470052)
  \drawline(3.4,0.34641012)(2.34641016,0.95470052)
  \end{picture}}}
\newcommand{\negtensorb}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,3.4641016){\makebox(0,0){$ #2 $}}  
  \put(4,3.4641016){\makebox(0,0){$ #3 $}}
  \put(2,2.3094011){\circle{.8}}
  \put(2,2.30940111){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(0.6,3.1176915)(1.6535989,2.5094011)
  \drawline(3.4,3.1176915)(2.34641016,2.5094011)
  \end{picture}}}
\newcommand{\tensorcu}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#3}} }
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \put(2,1.7320508){\circle{.8}}
  \put(2,1.7320508){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,0.8)(2,1.3320508)
  \drawline(2,2.1320508)(2,2.6641016)
  \end{picture}}}
\newcommand{\tensorunita}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(2,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \put(2,1.7320508){\circle{.8}}
  \put(2,1.7320508){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,2.1320508)(2,2.6641016)
  \end{picture}}}
\newcommand{\tensorunitb}[2]{%
\mbox{%
  \begin{picture}(4,4)
  \put(2,0){\makebox(0,0){\ensuremath{#2}} }
  \put(2,1.7320508){\circle{.8}}
  \put(2,1.7320508){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
  \drawline(2,0.8)(2,1.3320508)
  \end{picture}}}

\newcommand{\ltensor}[3]{%
   \partopcenter{[L\otimes]}{#1}{#2}{#3}}
\newcommand{\rtensor}[3]{%
   \tensorbottomcenter{[R\otimes]}{#1}{#2}{#3}}
\newcommand{\lbullet}[3]{%
   \partopcenter{[L\bullet]}{#1}{#2}{#3}}
\newcommand{\rbullet}[3]{%
   \tensorbottomcenter{[R\bullet]}{#1}{#2}{#3}}
\newcommand{\rdiamond}[2]{%
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \put(0,0){\makebox(0,0){\ensuremath{#1}} }
  \put(0.8,1.7320508){\makebox(0,0){\ensuremath{\scriptstyle [R\Diamond]}}}
  \drawline(0,0.8)(0,2.6641016)}
\newcommand{\ldiamond}[2]{%
  \put(0,3.4641016){\makebox(0,0){\ensuremath{#2}} }
  \put(0,0){\makebox(0,0){\ensuremath{#1}} }
  \put(0.8,1.7320508){\makebox(0,0){\ensuremath{\scriptstyle [L\Diamond]}}}
  \dottedline{.\thedotfactor}(0,0.8)(0,2.6641016)}
\newcommand{\lpar}[3]{%
   \tensortopcenter{[L\prs]}{#1}{#2}{#3}}
\newcommand{\rpar}[3]{%
   \parbottomcenter{[R\prs]}{#1}{#2}{#3}}
\newcommand{\limpl}[3]{%
   \tensortopleft{[L\lolli]}{#3}{#1}{#2}}
\newcommand{\rimpl}[3]{%
   \parbottomleft{[R\lolli]}{#3}{#1}{#2}}
\newcommand{\lldl}[3]{%
   \tensortopright{[L\backslash]}{#2}{#1}{#3}}
\newcommand{\lrdl}[3]{%
   \parbottomright{[R\backslash]}{#2}{#1}{#3}}
\newcommand{\lldr}[3]{%
   \tensortopleft{[L/]}{#1}{#3}{#2}}
\newcommand{\lrdr}[3]{%
   \parbottomleft{[R/]}{#1}{#3}{#2}}

\newcommand{\timeslink}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \drawline(2.4,1)(3.9,3)
  \drawline(1.6,1)(0.1,3)
  \end{picture}}}
\newcommand{\leftlink}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(4,4){\makebox(0,0){$ #3 $} }
  \put(2,0){\makebox(0,0){$ #1 $} }
  \drawline(1.6,1)(0.1,3)
  \end{picture}}}
\newcommand{\rightlink}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(4,4){\makebox(0,0){$ #3 $} }
  \put(2,0){\makebox(0,0){$ #1 $} }
  \drawline(2.4,1)(3.9,3)
  \end{picture}}}

\newcommand{\parlink}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \dottedline{.2}(2.4,1)(3.9,3)
  \dottedline{.2}(1.6,1)(0.1,3)
  \qbezier(2.4,1)(2,1.5)(1.6,1)
  \end{picture}}}

\newcommand{\cparlink}[4]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #3 $} }  
  \put(4,4){\makebox(0,0){$ #4 $} }  
  \put(2,0){\makebox(0,0){$ #2 $} }
  \textcolor{#1}{
  \dottedline{.2}(2.4,1)(3.9,3)
  \dottedline{.2}(1.6,1)(0.1,3)
  \qbezier(2.4,1)(2,1.5)(1.6,1)}
  \end{picture}}}

\newcommand{\unarylink}[2]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(0,0){\makebox(0,0){$ #1 $} }
  \drawline(0,1)(0,3)
  \end{picture}}}

\newcommand{\unarylinksub}[3]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(0,0){\makebox(0,0){$ #1 $} }
  \put(0.3,2){\makebox(0,0)[l]{$\scriptstyle [#3]$}}
  \drawline(0,1)(0,3)
  \end{picture}}}

\newcommand{\unaryparlink}[2]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(0,0){\makebox(0,0){$ #1 $} }
  \dottedline{.2}(0,1)(0,3)
  \end{picture}}}    

\newcommand{\trlprod}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(2.4,1){\vector(2,3){1.3}}
  \put(1.6,1){\vector(-2,3){1.3}}
  \end{picture}}}

\newcommand{\trrprod}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(3.7,2.9){\vector(-2,-3){1.3}}
  \put(0.3,2.9){\vector(2,-3){1.3}}
  \end{picture}}}

\newcommand{\trldr}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(1.6,1){\vector(-2,3){1.3}}
  \end{picture}}}

\newcommand{\trldl}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(2.4,1){\vector(2,3){1.3}}
  \end{picture}}}

\newcommand{\trldra}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(1.6,1){\vector(-2,3){1.3}}
  \put(2.8,3.6){\vector(-1,0){1.6}}
  \end{picture}}}

\newcommand{\trldla}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(2.4,1){\vector(2,3){1.3}}
  \put(1.2,3.6){\vector(1,0){1.6}}
  \end{picture}}}

\newcommand{\trrdr}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(0.3,2.9){\vector(2,-3){1.3}}
  \end{picture}}}

\newcommand{\trrdl}[3]{%
\mbox{%
  \begin{picture}(4,4)
  \put(0,4){\makebox(0,0){$ #2 $} }  
  \put(4,4){\makebox(0,0){$ #3 $} }  
  \put(2,0){\makebox(0,0){$ #1 $} }
  \put(3.7,2.9){\vector(-2,-3){1.3}}
  \end{picture}}}

\newcommand{\trdown}[2]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(0,0){\makebox(0,0){$ #1 $} }
  \put(0,3){\vector(0,-1){2}}
  \end{picture}}}

\newcommand{\trup}[2]{%
\mbox{%
  \begin{picture}(0,4)
  \put(0,4){\makebox(0,0){$ #2 $} }
  \put(0,0){\makebox(0,0){$ #1 $} }
  \put(0,1){\vector(0,1){2}}
  \end{picture}}}

\newcommand{\xnode}[3]{\ensuremath{\overset{#1}{\underset{#2}{\ensuremath{x_{#3}}}}}}
\newcommand{\node}[2]{\ensuremath{\overset{#1}{\underset{#2}{\makebox[1ex][c]{\rule{0ex}{1.2ex}\smash{\raisebox{.6ex}{\ensuremath{\centerdot}}}}}}}}
\newcommand{\nnode}[2]{\begin{picture}(0,0)
\put(0,0.12){\makebox(0,0){\ensuremath{\centerdot}}}%
\put(0,0.4){\makebox(0,0)[b]{\ensuremath{\scriptstyle #1}}}%
\put(0,-0.6){\makebox(0,0)[t]{\ensuremath{\scriptstyle #2}}}%
\end{picture}}
\newcommand{\anode}[2]{\begin{picture}(0,0)
\put(0,0.12){\makebox(0,0){\ensuremath{\centerdot}}}%
\put(0,0.25){\makebox(0,0)[b]{\ensuremath{\scriptstyle #1}}}%
\put(0,-0.3){\makebox(0,0)[t]{\ensuremath{\scriptstyle #2}}}%
\end{picture}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
%
% als labels bij de derivaties
%
\newcommand{\axn}{\textsc{\footnotesize Ax}}
\newcommand{\cutn}{\textsc{\footnotesize Cut}}
\newcommand{\strn}{\textsc{\footnotesize Struct}}
%
% connectieven
%    m multiplicatief
%    a additief
%    u unair
%
\newcommand{\mand}{\mathbin{\bullet}}		% times
\newcommand{\sand}[1]{\mathbin{\,\circ_{#1}\,}} % bijbehorende structuur *
%
\newcommand{\uand}{\mathord{\Diamond}}
\newcommand{\br}[2]{\langle #2 \rangle^{#1}} % bijbehorende structuur ^
%
\newcommand{\uor}{\mathord{\Box^{\downarrow}}}
\newcommand{\mim}{\mathbin{\backslash}}          % linear implication
\newcommand{\mimb}{\mathbin{/}}		% linear implication back
%
% voor stellingen/lemma's enz.  en  bewijzen.
%
\newcommand{\hhfill}{\ \ \ \vspace{-\baselineskip}\mbox{}\\ \mbox{}\hfill}
\newcommand{\ruitje}{\hhfill $\blacklozenge$}   % einde stelling/lemma
%
% proof structure macroos
%
\newcommand{\pijlbovendown}{%
	\begin{picture}(0,0)(0,0)
	\drawline(0,1)(0,.4)(-.2,.6)(0,.4)(.2,.6)
	\end{picture}} % boven formule en omlaag
\newcommand{\lijnbovendown}{%
	\begin{picture}(0,0)(0,0)
	\drawline(0,1)(0,.4)
	\end{picture}} % boven formule en omlaag
\newcommand{\pijlbovenup}{%
	\begin{picture}(0,0)(0,0)
	\drawline(0,1)(0,.6)(-.2,.4)(0,.6)(.2,.4)
	\end{picture}} % boven formule en omhoog
\newcommand{\pijlonderdown}{%
	\begin{picture}(0,0)(0,0) 
	\drawline(0,-1)(0,-.6)(-.2,-.4)(0,-.6)(.2,-.4) 
	\end{picture}} % onder formule en omlaag
\newcommand{\pijlonderup}{%
	\begin{picture}(0,0)(0,0)   
	\drawline(0,-1)(0,-.4)(-.2,-.6)(0,-.4)(.2,-.6) 
	\end{picture}} % onder formule en omhoog
\newcommand{\lijnonderdown}{%
	\begin{picture}(0,0)(0,0) 
	\drawline(0,-1)(0,-.4)
	\end{picture}} % onder formule en omlaag
\newcommand{\pijlpremisse}{%
	\begin{picture}(0,0)(0,0)
	\drawline(0,0.8)(0,.6)(-.2,.4)(0,.6)(.2,.4)
	\end{picture}} % boven formule en omhoog
\newcommand{\pijlconclusion}{%
	\begin{picture}(0,0)(0,0) 
	\drawline(0,-0.8)(0,-.6)(-.2,-.4)(0,-.6)(.2,-.4) 
	\end{picture}} % onder formule en omlaag

\newcommand{\wordbox}[2]{\makebox(0,0)[#1]{\fbox{\rule{0pt}{0.8em}$\smash{\text{#2}}_{\rule{0pt}{1ex}}$}}}

\newcommand{\cvanboven}[4]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\pijlbovendown} 
\put(0,1){\line(0,1){#2}} 
\put(0,#2){\begin{picture}(0,0)(0,0)\color[gray]{#4}{\put(0,1){\filltype{shade}\circle*{.3}\filltype{black}}\put(0,1.3){\makebox(0,0)[b]{{\tiny\raisebox{-.2ex}[0pt][0pt]{\textnormal{\color[gray]{#4}{R$ #3 $}}}}}}}\end{picture}}  
\end{picture}}}

\newcommand{\vanboven}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\pijlbovendown} 
\put(0,1){\line(0,1){#2}} 
\put(0,#2){\begin{picture}(0,0)(0,0)\put(0,1){\circle*{.3}}\put(0,1.3){\makebox(0,0)[b]{{\tiny\raisebox{-.2ex}[0pt][0pt]{\textnormal{R$ #3 $}}}}}\end{picture}}  
\end{picture}}}

\newcommand{\hvanboven}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\lijnbovendown}
\put(0,1){\line(0,1){#2}} 
\put(0,#2){\begin{picture}(0,0)(0,0)
	\put(0,1){\circle{.3}} 
	\put(0,1.3){\makebox(0,0)[b]{{\;\,\tiny\raisebox{-.2ex}[0pt][0pt]{\textnormal{$ #3 $}}}}}
	\end{picture}}  
\end{picture}}}

\newcommand{\naarboven}[2]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\pijlbovenup} 
\put(0,1){\line(0,1){#2}} 
\put(0,#2){\begin{picture}(0,0)(0,0) \put(0,1){\circle{.3}} \end{picture}}  
\end{picture}}}

\newcommand{\leegboven}[2]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\drawline(0,1)(0,.4) 
\put(0,1){\line(0,1){#2}} 
\put(0,#2){\begin{picture}(0,0)(0,0) \put(0,1){\circle{.3}} \end{picture}}  
\end{picture}}}

\newcommand{\naaronder}[2]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\pijlonderdown} 
\put(0,-1){\line(0,-1){#2}} 
\put(0,-#2){\begin{picture}(0,0)(0,0) \put(0,-1){\circle{.3}} \end{picture}}  
\end{picture}}}

\newcommand{\hnaaronder}[2]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\lijnonderdown} 
\put(0,-1){\line(0,-1){#2}} 
\put(0,-#2){\begin{picture}(0,0)(0,0) \put(0,-1){\circle{.3}} \end{picture}}  
\end{picture}}}


\newcommand{\vanonder}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\pijlonderup} 
\put(0,-1){\line(0,-1){#2}} 
\put(0,-#2){\begin{picture}(0,0)(0,0) \put(0,-1){\circle*{.3}} \put(0,-1.3){\makebox(0,0)[b]{{\tiny\raisebox{-1.4ex}[0pt][0pt]{\textnormal{L$ #3 $}}}}} \end{picture}}  
\end{picture}}}

\newcommand{\gvanonder}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{\ensuremath{#1}}}}
\put(0,0){\color[gray]{0.5}{\pijlonderup}} 
\put(0,-1){\line(0,-1){#2}} 
\put(0,-#2){\begin{picture}(0,0)(0,0)
            \put(0,-1){\filltype{shade}\color[gray]{0.5}{\circle*{.3}}\filltype{black}}
            \put(0,-1.3){\makebox(0,0)[b]{\tiny\raisebox{-1.4ex}[0pt][0pt]{\textnormal{\color[gray]{0.5}{L$ #3 $}}}}}
            \end{picture}}  
\end{picture}}}

\newcommand{\naaronderp}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{$ #1 $}}}
\put(0,0){\pijlonderdown}
\put(0,0){\pijlpremisse}
\put(0,0.8){\wordbox{b}{#3}}
\put(0,-1){\line(0,-1){#2}} 
\put(0,-#2){\begin{picture}(0,0)(0,0) \put(0,-1){\circle{.3}} \end{picture}}  
\end{picture}}}

\newcommand{\vanonderp}[4]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{$ #1 $}}}
\put(0,0){\pijlonderup}
\put(0,0){\pijlpremisse} 
\put(0,0.8){\wordbox{b}{#4}}
\put(0,-1){\line(0,-1){#2}} 
\put(0,-#2){\begin{picture}(0,0)(0,0)
	\put(0,-1){\circle*{.3}}
	\put(0,-1.3){\makebox(0,0)[b]{{\tiny\raisebox{-.8ex}[0pt][0pt]{\textnormal{L$ #3 $}}}}}
	\end{picture}}
\end{picture}}}

\newcommand{\hnaaronderp}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{$ #1 $}}}
\put(0,0){\lijnonderdown}
\put(0,0){\pijlpremisse} 
\put(0,0.8){\wordbox{b}{#3}}
\put(0,-1){\line(0,-1){#2}} 
\end{picture}}}

\newcommand{\hardelink}[1]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\drawline(0,0)(#1,0) 
\end{picture}}}

\newcommand{\zachtelink}[1]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\dashline[+60]{.25}(0,0)(#1,0) 
\end{picture}}}

\newcommand{\hardelinkx}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\drawline(0,0)(#1,0) 
\end{picture}}%
\makebox[0pt]{\begin{picture}(0,0)(-.0,-1.08)%
{\tiny\begin{tabular}{CCCCCCCCCCCCCCCCCCC}
#2
\end{tabular}}\end{picture}}%
\makebox[0pt]{\begin{picture}(0,0)(-.0,-.54)%
{\tiny\begin{tabular}{CCCCCCCCCCCCCCCCCCC}
#3
\end{tabular}}\end{picture}}
}

\newcommand{\zachtelinkx}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\dashline[+60]{.25}(0,0)(#1,0) 
%\put(0,0){\line(1,0){#1}}
\end{picture}}%
\makebox[0pt]{\begin{picture}(0,0)(-.0,-1.08)%
{\tiny\begin{tabular}{CCCCCCCCCCCCCCCCCCC}
#2
\end{tabular}}\end{picture}}%
\makebox[0pt]{\begin{picture}(0,0)(-.0,-.54)%
{\tiny\begin{tabular}{CCCCCCCCCCCCCCCCCCC}
#3
\end{tabular}}\end{picture}}
}

\newcommand{\tbranch}[5]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(0,0){\makebox(0,0){#3}}
  \put(2,0){\makebox(0,0){#4}}
  \put(4,0){\makebox(0,0){#5}}
  \drawline(0.6,0.6)(1.7,1.7)
  \drawline(3.4,0.6)(2.3,1.7)
  \drawline(2,1.6)(2,0.6)
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranch}[4]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(0,0){\makebox(0,0){#3}}
  \put(4,0){\makebox(0,0){#4}}
  \drawline(0.6,0.6)(1.7,1.7)
  \drawline(3.4,0.6)(2.3,1.7)
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranchau}[4]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(0,0){\makebox(0,0){#3}}
  \put(4,0){\makebox(0,0){#4}}
  \drawline(0.6,0.6)(1.7,1.7)
  \drawline(3.4,0.6)(2.3,1.7)
  \put(2,2.4){\vector(0,1){1}}
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranchal}[4]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(0,0){\makebox(0,0){#3}}
  \put(4,0){\makebox(0,0){#4}}
  \put(1.7,1.7){\vector(-1,-1){1}}
  \drawline(3.4,0.6)(2.3,1.7)
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranchar}[4]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(0,0){\makebox(0,0){#3}}
  \put(4,0){\makebox(0,0){#4}}
  \drawline(0.6,0.6)(1.7,1.7)
  \put(2.3,1.7){\vector(-1,1){1}}
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranchy}[4]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){\textcolor{yellow}{#2}}}%
  \put(0,0){\makebox(0,0){\textcolor{yellow}{#3}}}%
  \put(4,0){\makebox(0,0){\textcolor{yellow}{#4}}}%
  \textcolor{yellow}{\drawline(0.6,0.6)(1.7,1.7)}%
  \textcolor{yellow}{\drawline(3.4,0.6)(2.3,1.7)}%
  \textcolor{yellow}{\drawline(2,3.4)(2,2.4)}%
  \put(2,2){\textcolor{yellow}{\circle{0.8}}}%
  \put(2,2){\makebox(0,0){\ensuremath{\textcolor{yellow}{\scriptstyle #1}}}}
 \end{picture}
}
\newcommand{\bbranchlr}[3]{%
 \begin{picture}(4,4)
  \put(0,0){\makebox(0,0){#2}}
  \put(4,0){\makebox(0,0){#3}}
  \drawline(0.6,0.6)(1.7,1.7)
  \drawline(3.4,0.6)(2.3,1.7)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbrancht}[2]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranchl}[3]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(0,0){\makebox(0,0){#3}}
  \drawline(0.6,0.6)(1.7,1.7)
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\bbranchr}[3]{%
 \begin{picture}(4,4)
  \put(2,4){\makebox(0,0){#2}}
  \put(4,0){\makebox(0,0){#3}}
  \drawline(3.4,0.6)(2.3,1.7)
  \drawline(2,3.4)(2,2.4)
  \put(2,2){\circle{0.8}}
  \put(2,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\ubranch}[3]{%
 \begin{picture}(2,4)
  \put(1,4){\makebox(0,0){#2}}
  \put(1,0){\makebox(0,0){#3}}
  \drawline(1,0.6)(1,1.6)
  \drawline(1,2.4)(1,3.4)
  \put(1,2){\circle{0.8}}
  \put(1,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\ubranchbot}[2]{%
 \begin{picture}(2,4)
  \put(1,0){\makebox(0,0){#2}}
  \drawline(1,0.6)(1,1.6)
  \put(1,2){\circle{0.8}}
  \put(1,2){\makebox(0,0){\ensuremath{\scriptstyle #1}}}
 \end{picture}
}
\newcommand{\lbbranch}[3]{%
 \begin{picture}(4,3)
  \put(2,3){\makebox(0,0){#1}}
  \put(0,0){\makebox(0,0){#2}}
  \put(4,0){\makebox(0,0){#3}}
  \drawline(0.6,0.6)(1.7,2.4)
  \drawline(3.4,0.6)(2.3,2.4)
 \end{picture}
}
\newcommand{\lubranch}[2]{%
 \begin{picture}(2,3)
  \put(1,3){\makebox(0,0){#1}}
  \put(1,0){\makebox(0,0){#2}}
  \drawline(1,0.6)(1,2.4)
 \end{picture}
}
\newcommand{\tbt}[5]{%
 \begin{picture}(4,4)
   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(3.4,3.4)(2.3,2.3)
   \drawline(2,2.4)(2,3.4)
   \put(2,1.6){\vector(0,-1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(2,4){\makebox(0,0){#4}}
   \put(4,4){\makebox(0,0){#5}}
 \end{picture}
}
\newcommand{\tba}[5]{%
 \begin{picture}(4,4)
   \drawline(3.4,3.4)(2.3,2.3)
   \drawline(2,2.4)(2,3.4)
   \drawline(2,1.6)(2,0.6)
   \put(1.7,2.3){\vector(-1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(2,4){\makebox(0,0){#4}}
   \put(4,4){\makebox(0,0){#5}}
 \end{picture}
}
\newcommand{\tbb}[5]{%
 \begin{picture}(4,4)
   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(3.4,3.4)(2.3,2.3)
   \drawline(2,1.6)(2,0.6)
   \put(2,2.4){\vector(0,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(2,4){\makebox(0,0){#4}}
   \put(4,4){\makebox(0,0){#5}}
 \end{picture}
}
\newcommand{\tbc}[5]{%
 \begin{picture}(4,4)
   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(2,2.4)(2,3.4)
   \drawline(2,1.6)(2,0.6)
   \put(2.3,2.3){\vector(1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(2,4){\makebox(0,0){#4}}
   \put(4,4){\makebox(0,0){#5}}
 \end{picture}
}
\newcommand{\lprod}[4]{%
 \begin{picture}(4,4)
   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(3.4,3.4)(2.3,2.3)
   \put(2,1.6){\vector(0,-1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(4,4){\makebox(0,0){#4}}
 \end{picture}
}
\newcommand{\ldia}[3]{%
 \begin{picture}(2,4)
  \drawline(1,2.4)(1,3.4)
  \put(1,1.6){\vector(0,-1){1}}
  \filledcircle{1}{2}{.8}
   \circleindex{1}{2}{\scriptstyle #1}
   \put(1,2){\circle{.8}}
  \put(1,0){\makebox(0,0){#2}}
  \put(1,4){\makebox(0,0){#3}}
 \end{picture}
}
\newcommand{\rdr}[4]{%
 \begin{picture}(4,4)
   \drawline(3.4,3.4)(2.3,2.3)
   \drawline(2,0.6)(2,1.6)
   \put(1.7,2.3){\vector(-1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(4,4){\makebox(0,0){#4}}
 \end{picture}
}
\newcommand{\rdry}[4]{%
 \begin{picture}(4,4)
   \drawline(3.4,3.4)(2.3,2.3)
   \drawline(2,0.6)(2,1.6)
   \put(1.7,2.3){\vector(-1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\textcolor{yellow}{\scriptstyle #1}}
   \put(2,2){\textcolor{yellow}{\circle{.8}}}
   \put(2,0){\makebox(0,0){\textcolor{yellow}{#2}}}
   \put(0,4){\makebox(0,0){\textcolor{yellow}{#3}}}
   \put(4,4){\makebox(0,0){\textcolor{yellow}{#4}}}
 \end{picture}
}
\newcommand{\rdrb}[4]{%
 \begin{picture}(4,4)
%   \drawline(3.4,3.4)(2.3,2.3)
   \drawline(2,0.6)(2,1.6)
   \put(1.7,2.3){\vector(-1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(4,4){\makebox(0,0){#4}}
 \end{picture}
}
\newcommand{\rdl}[4]{%
 \begin{picture}(4,4)
   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(2,0.6)(2,1.6)
   \put(2.3,2.3){\vector(1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(4,4){\makebox(0,0){#4}}
 \end{picture}
}
\newcommand{\rdly}[4]{%
 \begin{picture}(4,4)
   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(2,0.6)(2,1.6)
   \put(2.3,2.3){\vector(1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\textcolor{yellow}{\scriptstyle #1}}
   \put(2,2){\textcolor{yellow}{\circle{.8}}}
   \put(2,0){\makebox(0,0){\textcolor{yellow}{#2}}}
   \put(0,4){\makebox(0,0){\textcolor{yellow}{#3}}}
   \put(4,4){\makebox(0,0){\textcolor{yellow}{#4}}}
 \end{picture}
}
\newcommand{\rdlb}[4]{%
 \begin{picture}(4,4)
%   \drawline(0.6,3.4)(1.7,2.3)
   \drawline(2,0.6)(2,1.6)
   \put(2.3,2.3){\vector(1,1){1.1}}
   \filledcircle{2}{2}{.8}
   \circleindex{2}{2}{\scriptstyle #1}
   \put(2,2){\circle{.8}}
   \put(2,0){\makebox(0,0){#2}}
   \put(0,4){\makebox(0,0){#3}}
   \put(4,4){\makebox(0,0){#4}}
 \end{picture}
}
\newcommand{\rbox}[3]{%
 \begin{picture}(2,4)
  \put(1,2.4){\vector(0,1){1}}
  \drawline(1,1.6)(1,0.6)
   \filledcircle{1}{2}{.8}
   \circleindex{1}{2}{\scriptstyle #1}
   \put(1,2){\circle{.8}}
   \put(1,0){\makebox(0,0){#2}}
   \put(1,4){\makebox(0,0){#3}}
 \end{picture}
}

\newcommand{\terminal}[1]{%
\makebox(0,0){\normalsize\raisebox{-1.1em}{\fbox{\rule{0pt}{0.66em}$\smash{\textup{#1}}_{\rule{0pt}{0.5ex}}$}}}
}

\newcommand{\simplelex}[2]{%
 \begin{picture}(0,2)
  \put(0,2){\makebox(0,0){#2}}
  \put(0,0){\terminal{#1}}
  \drawline(0,0.6)(0,1.4)
 \end{picture}
}
\newcommand{\simplelexb}[2]{%
 \begin{picture}(0,2.0)
  \put(0,2.0){\makebox(0,0){#2}}
  \put(0,-0.4){\terminal{#1}}
  \path(0,0.2)(0,1.4)
 \end{picture}
}
\newcommand{\simpleaps}[2]{%
 \begin{picture}(0,2)
  \put(0,2){\makebox(0,0){\ensuremath{\scriptstyle #2}}}
  \put(0,0){\terminal{#1}}
  \put(0,1.25){\nnode{}{}}
 \end{picture}}
\newcommand{\apsterminal}[1]{%
 \begin{picture}(0,0)
  \put(0,0){\nnode{}{}}
  \put(0,-1.25){\terminal{#1}}
 \end{picture}}
\newcommand{\apsterminalx}[2]{%
 \begin{picture}(0,0)
  \put(0,0){\nnode{#2}{}}
  \put(0,-1.25){\terminal{#1}}
 \end{picture}}

% = pages

\newcommand{\sk}[1]{%
\vspace{#1\baselineskip}
}

\newcommand{\ant}[1]{\ensuremath{\stackrel{-}{#1}}}
\newcommand{\suc}[1]{\ensuremath{\stackrel{+}{#1}}}
\newcommand{\neut}[1]{\ensuremath{\stackrel{.}{#1}}}

\newcommand{\ants}[1]{\stackrel{-}{\scriptstyle #1}}
\newcommand{\sucs}[1]{\stackrel{+}{\scriptstyle #1}}
\newcommand{\neuts}[1]{\stackrel{.}{\scriptstyle #1}}

\newcommand{\redone}{\ensuremath{\stackrel{1}{\rightarrow}}}
\newcommand{\redtwo}{\ensuremath{\stackrel{2}{\rightarrow}}}
\newcommand{\redx}[1]{\ensuremath{\stackrel{#1}{\rightarrow}}}

\newcommand{\rf}[1]{\raisebox{.23ex}{#1}}

\newcommand{\appl}[2]{(#1\ #2)}
\newcommand{\lolli}{\mbox{$\mathbin{- \!\circ}$}}
\newcommand{\blolli}{\mbox{$\mathbin{\circ\! -}$}}
\newcommand{\cololli}{\mbox{$- \!\bullet$}}
\newcommand{\bcololli}{\mbox{$\bullet\! -$}}

\newcommand{\pr}{ \mathbin{\smash{\raisebox{1.6ex}{\begin{turn}{-180}{\ensuremath{\&}}\end{turn}}}}}
\newcommand{\prscript}{ \mathbin{\smash{\raisebox{0.8ex}{\begin{turn}{-180}{\ensuremath{\scriptstyle{\&}}}\end{turn}}}}}
\newcommand{\prx}{\mathbin{\begin{turn}{-180}\ensuremath{\&}\end{turn}}}
\newcommand{\prs}{ \smash{\raisebox{1.15ex}{\begin{turn}{-180} \ensuremath{\scriptstyle\&} \end{turn}}}}
\newcommand{\dv}{\!:\!}

\newcommand{\set}[1]{\ensuremath{\{ #1 \} }}

\newcommand{\longpage}{\enlargethispage{\baselineskip}}
\newcommand{\shortpage}{\enlargethispage{-\baselineskip}}

%\newcommand{\proof}{\textbf{Proof}\ }


\newcommand{\ralabel}[2]{\makebox[2.5em]{$\mathbin{\stackrel{\text{$#1$}}{\rightarrow}_{\text{$#2$}}}$}}
\newcommand{\lalabel}[2]{\makebox[2.5em]{$\mathbin{\stackrel{\text{$#1$}}{\leftarrow}_{\text{$#2$}}}$}}

\newcommand{\thralabel}[2]{\makebox[2.5em]{$\mathbin{\stackrel{\text{$#1$}}{\twoheadrightarrow}_{\text{$#2$}}}$}}

\newcommand{\Rl}[1]{\RL{#1}}
\newcommand{\frakps}{\ensuremath{\mathcal{PS}}}
\newcommand{\fCenter}{\;\vdash_{\rule{0pt}{1ex}}\;}
\newcommand{\dddots}{\mathpunct{%
	\begin{sideways} 
	\textnormal{$\ddots$}
	\end{sideways}}}		
\newcommand{\pstoaps}{\mapsto}

\newcommand{\svanboven}[3]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines 
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{$ #1 $}}}
\put(0,0){\pijlbovendown} 
\put(0,1){\line(0,1){#2}} 
\put(0,#2){\begin{picture}(0,0)(0,0)
	\put(0,1){\circle*{.3}} 
	\put(0,1.4){\makebox(0,0)[b]{{\tiny\raisebox{-.8ex}[0pt][0pt]{\textnormal{$ #3 $}}}}}
	\end{picture}}  
\end{picture}}}

\newcommand{\equals}[2]{\makebox[2.5em]{$\mathbin{\stackrel{\text{$#1$}}{=\!\!=}_{\text{$#2$}}}$}}

\newcommand{\norm}[1]{\left|\!\left| #1 \right|\!\right|}

\newcommand{\nodes}[2]{\overset{\text{$#1$}}{\underset{\text{$#2$}}{\node{}{}\;\node{}{}\;\node{}{}}}}

\newcommand{\delete}[1]{}

\newcommand{\ovaalb}{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\put(0,0){\oval(2.5,1.25)[b]} 
\end{picture}}}

\newcommand{\ovaalt}{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\thicklines
\put(0,0){\oval(2.5,1.25)[t]} 
\end{picture}}}

\newcommand{\hier}[1]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\put(0,0){\makebox(0,0)[b]{\raisebox{-.8ex}[0pt][0pt]{$ #1 $}}}
\end{picture}}
}
\newcommand{\boven}[1]{\makebox[0pt]{\begin{picture}(0,0)(-.5,-.5)
\put(0,0){\makebox(0,0)[b]{\raisebox{-.2ex}[0pt][0pt]{$ #1 $}}}
\end{picture}}
}
\newcommand{\cala}{\mathcal{A}}
\newcommand{\calb}{\mathcal{B}}
\newcommand{\calc}{\mathcal{C}}
\newcommand{\cald}{\mathcal{D}}
\newcommand{\cale}{\mathcal{E}}
\newcommand{\calf}{\mathcal{F}}
\newcommand{\calg}{\mathcal{G}}
\newcommand{\calh}{\mathcal{H}}
\newcommand{\cali}{\mathcal{I}}
\newcommand{\calj}{\mathcal{J}}
\newcommand{\calk}{\mathcal{K}}
\newcommand{\call}{\mathcal{L}}
\newcommand{\calm}{\mathcal{M}}
\newcommand{\caln}{\mathcal{N}}
\newcommand{\calo}{\mathcal{O}}
\newcommand{\calp}{\mathcal{P}}
\newcommand{\calq}{\mathcal{Q}}
\newcommand{\calr}{\mathcal{R}}
\newcommand{\cals}{\mathcal{S}}
\newcommand{\calt}{\mathcal{T}}
\newcommand{\calu}{\mathcal{U}}
\newcommand{\calv}{\mathcal{V}}
\newcommand{\calw}{\mathcal{W}}
\newcommand{\calx}{\mathcal{X}}
\newcommand{\caly}{\mathcal{Y}}
\newcommand{\calz}{\mathcal{Z}}

%\newcommand{\ts}{\fCenter}
\newcommand{\llabel}[1]{\label{#1}}
\newcommand{\taud}{\tau_d}
\newcommand{\tauinv}{\tau^{-1}}

